Muscles in Time: Learning to Understand Human Motion by Simulating Muscle Activations

Exploring the intricate dynamics between muscular and skeletal structures is pivotal for understanding human motion. This domain presents substantial challenges, primarily attributed to the intensive resources required for acquiring ground truth muscle activation data, resulting in a scarcity of datasets. In this work, we address this issue by establishing Muscles in Time (MinT), a large-scale synthetic muscle activation dataset. For the creation of MinT, we enriched existing motion capture datasets by incorporating muscle activation simulations derived from biomechanical human body models using the OpenSim platform, a common approach in biomechanics and human motion research. Starting from simple pose sequences, our pipeline enables us to extract detailed information about the timing of muscle activations within the human musculoskeletal system. Muscles in Time contains over nine hours of simulation data covering 227 subjects and 402 simulated muscle strands. We demonstrate the utility of this dataset by presenting results on neural network-based muscle activation estimation from human pose sequences with two different sequence-to-sequence architectures. Data and code are provided under https://simplexsigil.github.io/mint.

==> sections/llm_baselines.tex <==
\subsection{Explorative usage of LLMs}
\begin{itemize}[label={-}]
    \item \david{David}, \simon{Simon}, \marco{Marco: \textbf{Inference of LLM}}
        \begin{itemize}[label={-}]
            \item \textbf{Use language annotations from Simon}: Label, Pose?, Muscle Annot. Question -> Answer
        \end{itemize} 
\end{itemize}

==> sections/notes.tex <==

\section{Simon's thoughts on experiments}

\subsection{Where do we want to go: Contribution and impact}

\begin{itemize}
    \item \underline{Dataset}: We are the first to make available a dataset which has quadruplets $(p_t, m_t, l, q, a)$ of temporal human pose trajectories, temporal fine-grained muscular activation, activity label, text questions regarding pose and muscles, answer to the question regarding pose and muscles.
    \item \underline{pose-to-muscular activation estimation} Direct pose-to-muscular activation estimation network \david{Show results for own data, compare with muscles in action}
    \item \underline{MuscleLLM} A trained, \underline{fine-tuned LLM} which can process pose trajectory data and a question about it as input and generate a textual answer.
\end{itemize}

\subsection{What do we need to report: Evaluation and results}
\textbf{Regarding the dataset contribution}
\begin{itemize}
    \item Dataset statistics on size, label distribution, muscular activation distribution, maybe co-occurrence of muscle activations
    \item Qualitative template question-answer examples \david{Hand crafted templates, possibly ask sports people for help?}
    \item Qualitative expert assessment
\end{itemize}

\textbf{Pose-to-muscular activation estimation contribution}
\begin{itemize}
    \item Quantitative prediction evaluation (metric: MSE?)
    \item Baselines, this can simply be different pose-processing network architectures, better: simple approaches from literature
\end{itemize}

\textbf{Regarding LLM contribution}
\begin{itemize}
    \item Quantitative evaluation of LLM capability to correctly answer: BLEU score, comparison to basline e.g. PoseGPT~\cite{feng2023posegpt} \david{Not yet available}, Video-GPT, maybe LLaVa~\cite{liu2023visual}. \david{Baselines similar to video LLM papers? Check if they also use these scores.}
    \item Pose-based activity inference by Question-answer pairs in the style of "Which activity is performed here" (metric: accuracy)
    \item (optional, cherry on top): Human expert eval: Preference evaluation of our LLM vs. a baseline of their generated answers given pose input \david{Use online network / service or run video gpt like model locally.}
    \item LLM, qualitative generation figure for ours + baseline
\end{itemize}

\subsection{What is still to be done: Work packages}
\begin{itemize}
    \item Compute muscle activation for rest of data (in progress, Marco) (Target: 31. of January if possible)
    \item Setup templates for question / answer generation (02. of February) \david{Use chat gpt for synonym generation and variations in templates} \simon{Simon}
    \item Generate full dataset with $(p_t, m_t, l, q, a)$ (06th of February)
    \item Setup dataloader for the dataset (07th of February)
    \item Train a pose-to-muscle activation model (14th February) \david{David} \kunyu{Kunyu}
    \item Evaluate pose-to-muscle model experiments (21st of February) \david{David} \kunyu{Kunyu}
    \item Select specific LLM for our work (e.g. PoseGPT like) (5th of February)
    \item Setup repository for LLM training (05th of February)
    \item Train adapter for pretrained LLM to include pose information (e.g. prefix tuning) + question text to produce answer text (16th February)
    \item implement script to evaluate LLM prediction (18th of February)
    \item Evaluate our LLM (23st of February)
    \item Write the paper (3rd of March)
\end{itemize}

Task examples:
\begin{itemize}
    \item Muscle to action: "Following muscles have been activated, what action is performed?
    \item Muscle to action: "Following muscles have been activated, what action is performed?
    \item Action to muscle: "I want to train my biceps, which action do I need to perform?"
    \item 
\end{itemize}



\iffalse
In this work, we rely on the AMASS dataset \cite{mahmood_amass_2019}. AMASS unifies the representation of marker-based mocap sequences with the MoSh++ method into standardized realistic human meshes in the format of SMPL skeletal respresentation.  The mocap data of AMASS includes marker-based optical human mocap data from several datasets, e.g. KIT, BMLrub and BMLmovi. With more than 11000 motions and 300 subjects, the dataset offers a comprehensive and exhaustive collection of human motion encompassing a wide spectrum of activities, ensuring thorough coverage of diverse movement patterns and behaviors. This enables the observation of a wide collection of different muscle activation patterns.

As the foundation of our muscle activation analysis serves the open-source tool OpenSim \cite{delp_opensim_2007}. OpenSim is a widely adopted tool within the community of biomechanical analysis. The strong collaboration of various researchers, practitioners and developers within OpenSim provide the necessary models, methods and tools to analyse muscle activation in the human movement. More specifically, the pipeline for our dataset generation uses the OpenSimAD~\cite{falisse_algorithmic_2019} implementation, similar to its use in the OpenCap \cite{uhlrich_opencap_2023} project. The implementation incorporates the capability of estimating the muscle activation without the explicitly measured Ground Reaction Forces~(GRF), which are usually measured in the context of biomechanical analysis with force plates. This force plate data is not part of the AMASS datasets, thus needs to be estimated.

OpenSimAD leverages algorithmic differentiation to solve the trajectory optimization problem with the kinematic data and the scaled musculoskeletal model. In order to further facilitate the analysis of human motion, we provide an approach of directly training a model on poses and the corresponding simulated muscle activation. The lightweight model has in contrast to the complex optimization problem advantages in terms of runtime, necessary computational power and usability. Our goal is not to replace, but to explore the option of further streamlining the existing OpenSim implementations to utilise it outside of the medical domain. 

The OpenSim process is based on the setting of markers on musculoskeletal models to scale the model subject-specific and follow the movements of the subject, i.e., the kinematic analysis. The pipeline incorporates the given musculoskeletal model of OpenCap for the leg muscles and a further validated and openly accessible model for the muscles in the thoracolumbar region, defined by Bruno et al. \cite{bruno_development_2015}. Muscles activations in the thoracolumbar model are analysed using the Static Optimization tool in OpenSim and the estimated GRF from the OpenCap optimization problem. The marker information in space and time is defined by specific indices of the AMASS body model, as can be seen on the left of figure \ref{fig:markersandmodels}. The utilized indices are those defined in the approach of Bittner at al. \cite{bittner_towards_2023}.

Our approach provides an automatic pipeline to generate simulated muscle activation data from the AMASS dataset and abstracts from the details of OpenSim and AMASS. With the published code, users can further iterate on the possibilities of analysing the biomechanics of the AMASS dataset with OpenSim.
\fi

==> sections/rebuttal.tex <==
\vspace{-6em}
\thispagestyle{nofooter}
Dear reviewers and chairs, we are thankful and appreciate the generally positive feedback on our work. We address the key questions and suggestions from \bfvp, \pwpd, \svhw, and \kybs in this global rebuttal, detailed responses will further be provided directly to the respective reviewers.

\noindent\textbf{Improved Documentation} \bfvp rightfully pointed out lacking documentation of the \href{https://github.com/simplexsigil/MusclesInTime}{MusclesInTime} repository. We added a detailed README and Jupyter notebooks for visualizing data samples including motion and intend to migrate this information to a readthedocs.io space.

\noindent\textbf{SMPL-H}
We acknowledge \bfvp 's concerns about SMPL-H motion quality, particularly for hands and feet. The AMASS dataset largely lacks hand articulation, so our muscle simulation omits related muscles, as shown in Figure 2. Unlike [9], which used VIBE for pose estimation, MinT's motions are based on high quality motion capture. This difference is evident in the animations linked below as well as in visualizations provided by the BABEL dataset: \href{https://human-movement.is.tue.mpg.de/explore/}{https://human-movement.is.tue.mpg.de/explore/}. Detailed marker visualization and used mesh vertex indices will shortly be added to the repository.

\noindent\textbf{Simulation quality and limitations} All reviewers acknowledged our efforts to list limitations which are unavoidable when using simulated data. \bfvp highlighted lines 119-122 where we mention that we follow the community in using pre-validated models, avoiding major changes. In line 128 we mention that we make use of Opensim's scaling mechanism, we means that we do scale the mass properties and body segment length to match an individuals anatomical properties. We will change the paper text to clarify this. We will also highlight the limitation of not adapting other model parameters such as muscle forces, raising awareness in future users of our dataset. The usage of pre-validated models is an important aspect of our simulation pipeline, specifically to address the lack of EMG ground truth recordings for verification in AMASS, significant changes to muscle geometry and properties would require an extensive per-individual re-validation using such recordings. \kybs inquires about quantitative evaluation of data quality. The optimization loss used in OpenSimAD which we use for muscle activation includes terms for position tracking, velocity, and acceleration errors as well as terms for activation minimization and reserve actuator minimization. While we do not make use of individual thresholds for these properties, we discard any results for which the optimization problem does not converge within the tolerance recommended by the the authors of OpenSimAD.

\noindent\textbf{Additional results and qualitative examples}
\svhw and \kybs suggested evaluation on further real world datasets. While Camargo \etal\ [4] and MiA [9] from Table 1 were the only viable options, Camargo \etal\ do not provide upper body motion capture points.
MiA provides only eight EMG measurement points, four of which align with our model. We tried mapping the hamstring measurement to the \emph{biceps femoris long head} and the quadriceps to the \emph{rectus femoris} muscle. Our main problem is that MiA motions are stationary, hovering above the ground and not aligning well with locomotion induced by the feet, making our model generalize badly due to its training on very precise AMASS motions. Fine-tuning on MiA was necessary, as presented in Table A5 in the supplementary. We plan to develop advanced domain adaptation methods to address these issues in future work. \kybs suggested additional baseline experiments. The T2M-GPT architecture was chosen for its effectiveness in generating useful intermediate representations for cross-modality translation tasks in human motion, making it a stronger baseline than arbitrary architectures. To address the request of \kybs, we are currently preparing additional baseline results which will be provided during the discussion period. To address \kybs' suggestion for showing predictions on MinT as well as for the model in Table A5 combined with the corresponding motion, we prepared two sets of videos containing animated movements with muscle activations and their respective predictions. These videos are available at \href{https://s.kit.edu/mint-vis}{https://s.kit.edu/mint-vis} for MinT and at \href{https://s.kit.edu/mia-vis}{https://s.kit.edu/mia-vis} for MiA. The jupyter notebooks used for generation can be found in the MinT repository.


\noindent\textbf{In-detail qualitative comparison}

To address the concerns of \kybs and \svhw regarding the simulation data quality and incorporation of real world data in more detail, we provide additional qualitative analysis on the animated motion and muscle activation data.
\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\linewidth]{imgs/mia_running_v2.png}
    \includegraphics[width=0.8\linewidth]{imgs/mint_running_v2.png}
    \caption{Real world EMG recordings from MiA (upper row) as well as simulated muscle activation values from MinT (lower row) on the activity \emph{running}.}
    \label{fig:mint_mia_comp_running}
\end{figure}
For this we prepared a comparison video which can be accessed under \href{https://s.kit.edu/mint-mia-comparison}{https://s.kit.edu/mint-mia-comparison}. An example is provided in Figure~\ref{fig:mint_mia_comp_running}. For each leg we marked the lowest compression point with dotted horizontal bars, the left leg from the avatars perspective is marked in blue, the right leg is marked in orange. We find the muscle activation peaks in MiA to be close the lowest compression points, with subject specific variations and a generally more noisy signal. MinT displays similar activation patterns, although the estimated activation is much more predictive and stable.

\noindent\textbf{Response to \svhw}
Thank you for your thoughtful feedback and suggestions for improvement. We appreciate your emphasis on the importance of comparing synthetic data to real-world EMG recordings, a concern we take seriously. As noted in our global rebuttal, comparing MinT to real-world data like MiA (Muscles in Action) presents challenges due to issues such as inaccurate pose estimation and subject-specific EMG recording noise. However, we have made efforts to address this in our work.

MiA is the most directly comparable real-world dataset to MinT. To facilitate a meaningful comparison, we have provided extensive animated motion sets with corresponding EMG values for both datasets. These animations allow for an in-depth qualitative analysis of EMG pattern similarities and the challenges of generalizing models trained on MinT. You can access the animations for MiA at \href{https://s.kit.edu/mia-vis}{https://s.kit.edu/mia-vis} and for MinT at \href{https://s.kit.edu/mint-vis}{https://s.kit.edu/mint-vis} (tar-files).

We have also created a detailed comparison of selected activity categories, available at \href{https://s.kit.edu/mint-mia-comparison}{https://s.kit.edu/mint-mia-comparison} (video). This comparison highlights the lowest compression points of each leg using blue and orange dotted vertical lines for the left and right legs, respectively. Our comparison shows that MiA exhibits significant noise and subject-specific scaling variations, while MinT demonstrates a more controlled and consistent pattern. This difference underscores the complexity of directly applying a model trained on MinT to MiA data, as MiA contains strong subject-specific characteristics. MiA itself does not provide a cross-subject split but rather allows a model to learn subject specific characteristics and exposes the model to the same subjects at test time. We believe that advanced domain generalization or adaptation techniques are necessary to achieve high performance with little or no training on the MiA target domain dataset. While this is an important area for future research, it extends beyond the scope of our current paper. We do, however, refer to the MiA fine-tuning experiment in Table A5 of the supplementary materials for additional context.

We also value your suggestion regarding the need for greater motion diversity in muscle activation datasets. Our dataset, as shown in the animations, offers a broad range of motion classes and significant intra-class diversity in motion execution, distinguishing it from the more controlled MiA dataset which is limited to a much smaller number of different activities. To our knowledge, MinT is the only dataset that combines such a diverse range of motions with detailed muscle activation data, making it uniquely valuable for a wide range of applications.

As suggested we will add a more detailed discussion of the limitations of synthetic data as well as comparisons between the motion patterns in MiA and MinT to the paper. Concerning the long-term implications, we believe that this dataset will incite further research on muscle activation focused machine learning. We see from MiA that EMG data varies significantly based on subject specifics and the recording setup, which is why we consider real-world data necessary for fine-tuning on down-stream tasks. We believe that MinT will have a significant impact as a pre-training dataset allowing a model to learn the clean characteristics of muscle activations. Adaptations to down-stream tasks might then either be made by using special generalization techniques like noise introduction in training or exposing the pre-trained model to real-world traing data during fine-tuning.

In response to your feedback, we will enhance our discussion of the limitations of synthetic data and include comparisons between MiA and MinT in the revised paper. Regarding the long-term implications, we believe MinT will play a significant role in advancing muscle activation-focused machine learning research. While real-world data will continue to be crucial for fine-tuning in downstream tasks, MinT serves as a critical pre-training dataset, enabling models to learn the clean characteristics of muscle activations. Future work might involve using techniques such as noise introduction during training or integrating real-world data during fine-tuning to adapt pre-trained models effectively.

We are committed to incorporating these improvements and believe they will significantly enhance the impact and relevance of our work.

\noindent\textbf{Response to \kybs}
Thank you for your thoughtful feedback and for bringing attention to several important areas for improvement in our work. We appreciate the opportunity to clarify and enhance our paper based on your comments.

Regarding the quantitative evaluation of data quality, as discussed in the global rebuttal, the optimization loss used in OpenSimAD includes terms for position tracking, velocity, and acceleration errors, as well as activation minimization and reserve actuator minimization. While we did not employ specific thresholds like the Hicks threshold, we ensured that any results where the optimization did not converge within the recommended tolerance were excluded from our dataset. We recognize the importance of further quantitative evaluation and are considering how to incorporate this in future work.

On the matter of baseline selection in Section 5, we chose the T2M-GPT architecture because of its effectiveness in generating intermediate representations for cross-modality translation tasks in human motion, which maintains similarities to our task, despite its differences. However, we acknowledge the value of comparing our approach to simpler models. In response to your suggestion, we are preparing additional baseline experiments and will provide them during this week.

You also suggested evaluating MinT-trained models on existing datasets from Table 1. We attempted to do this with MiA which is best suited to act as comparison, but MiA presents challenges due to issues such as inaccurate pose estimation and subject-specific EMG recording noise. Consequently, fine-tuning on MiA was necessary, as detailed in Table A5 of the supplementary materials and also mentioned in the response to reviewer 6vHW and the global rebuttal. We plan to explore advanced domain adaptation methods to address these challenges in future work.

We also agree with your suggestion to improve the clarity and structure of Sections 3 and 5. We will add subsection partitions to better organize the data processing and implementation details, including a clearer definition of the loss functions. These revisions should enhance the readability and comprehensibility of our paper.

In terms of related work, we will expand our discussion to include the studies you mentioned on musculoskeletal humanoid control and simulation. This will better situate our work within the broader field and highlight its relevance.

Finally, in response to your suggestion for qualitative result demonstration, we have prepared videos that showcase predictions on MinT, as well as on the model from Table A5, combined with the corresponding motion. These can be accessed at \href{https://s.kit.edu/mint-vis}{https://s.kit.edu/mint-vis} for MinT and \href{https://s.kit.edu/mia-vis}{https://s.kit.edu/mia-vis} for MiA. The Jupyter notebooks used to generate these videos are available in the MinT repository. Based on these animations we also provide a comparison video which can be accessed under \href{https://s.kit.edu/mint-mia-comparison}{https://s.kit.edu/mint-mia-comparison} (video) and demonstrates the similarities in activation patterns between MiA and MinT, despite the domain gap.

We are committed to incorporating these improvements and believe they will significantly enhance the quality and impact of our work. We appreciate your feedback and the opportunity to address these concerns in our revision.

==> tables/mot2mus_transabl.tex <==
{\addtolength{\tabcolsep}{-0.5em}
\begin{table}[h]
\centering
\caption{Human motion-to-muscle activation prediction results for the lower- and upper body model.}
\label{tab:motion-to-muscle_eval}
\begin{tabular}{@{}lccccccccc@{}}
\toprule
Motion  & \multicolumn{3}{c}{Transformer 4 Layer} & \multicolumn{3}{c}{Transformer 8 Layer} & \multicolumn{3}{c}{Transformer 16 Layer}\\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} 
& \small RMSE$\downarrow$ & \small SMAPE$\downarrow$ & \small PCC$\uparrow$ & \small RMSE$\downarrow$ & \small SMAPE$\downarrow$ & \small PCC$\uparrow$ & \small RMSE$\downarrow$ & \small SMAPE$\downarrow$ & \small PCC$\uparrow$ \\
\\[-1.5ex]
\multicolumn{10}{c}{\textit{Lower body model}} \\
\\[-1.5ex]
overall & 0.049  & 52.8 & 0.52 & \bst{0.048} & 49.1 & 0.53       & \bst{0.048} & \bst{45.1} & \bst{0.54}  \\
jump    & 0.051  & 57.2 & 0.69 & \bst{0.049} & 54.2 & \bst{0.71} & 0.051       & \bst{52.3} & \bst{0.71}  \\
kick    & 0.055  & 62.0 & 0.59 & 0.054       & 59.2 & 0.60       & \bst{0.053} & \bst{54.8} & \bst{0.62}  \\
stand   & 0.047  & 52.7 & 0.55 & \bst{0.046} & 48.8 & 0.56       & \bst{0.046} & \bst{45.0} & \bst{0.58}  \\
walk    & 0.046  & 50.5 & 0.74 & \bst{0.044} & 46.2 & 0.76       & \bst{0.044} & \bst{42.4} & \bst{0.77}  \\
jog     & 0.048  & 57.5 & 0.69 & \bst{0.046} & 55.2 & 0.70       & \bst{0.046} & \bst{51.1} & \bst{0.71}  \\
dance   & 0.059  & 64.2 & 0.64 & \bst{0.057} & 61.3 & 0.64       & \bst{0.057} & \bst{58.5} & \bst{0.65}  \\
\\[-1.5ex]
\multicolumn{10}{c}{\textit{Upper body model}} \\
\\[-1.5ex]
overall & 0.033       & 109.3 & 0.53 & \bst{0.032} & 108.4       & 0.54 & 0.033       & \bst{107.7} & \bst{0.55}  \\
jump    & 0.052       & 114.0 & 0.61 & \bst{0.051} & 112.8       & 0.62 & 0.052       & \bst{112.7} & \bst{0.63}  \\
kick    & 0.046       & 116.4 & 0.62 & 0.046       & 115.7       & 0.62 & \bst{0.044} & \bst{114.8} & \bst{0.65}  \\
stand   & 0.030       & 112.2 & 0.53 & 0.029       & 111.4       & 0.54 & \bst{0.028} & \bst{110.5} & \bst{0.55}  \\
walk    & \bst{0.019} & 103.9 & 0.61 & \bst{0.019} & 103.3       & 0.62 & \bst{0.019} & \bst{102.6} & \bst{0.63}  \\
jog     & 0.029       & 111.8 & 0.69 & \bst{0.028} & 111.2       & 0.70 & 0.029       & \bst{110.8} & \bst{0.71}  \\
dance   & 0.040       & 123.4 & 0.57 & \bst{0.034} & \bst{121.7} & 0.58 & 0.036       & 121.8       & \bst{0.59}  \\
\bottomrule
\end{tabular}
\end{table}
}

==> tables/results_mia.tex <==
Pretrainging Mint, 100\% data:

Scratch
Action & RMSE & PCorr & SMAPE
overall (3000) & 0.140 & 0.27 & 37.2
ElbowPunch (201) & 0.139 & 0.24 & 43.4
FrontKick (200) & 0.095 & 0.19 & 35.3
FrontPunch (213) & 0.080 & 0.39 & 30.0
HighKick (182) & 0.128 & 0.34 & 36.5
HookPunch (200) & 0.123 & 0.33 & 37.4
JumpingJack (200) & 0.122 & 0.27 & 28.8
KneeKick (188) & 0.129 & 0.25 & 37.1
LegBack (208) & 0.156 & 0.31 & 37.7
LegCross (182) & 0.125 & 0.17 & 43.0
RonddeJambe (220) & 0.151 & 0.23 & 39.0
Running (200) & 0.079 & 0.30 & 26.6
Shuffle (198) & 0.088 & 0.19 & 27.9
SideLunges (202) & 0.209 & 0.27 & 46.5
SlowSkater (201) & 0.195 & 0.26 & 42.7
Squat   (205) & 0.187 & 0.23 & 45.9
overall (3000) & 0.140 & 0.27 & 37.2


Pret
Action & RMSE & PCorr & SMAPE
overall (3000) & 0.140 & 0.27 & 37.3
ElbowPunch (201) & 0.139 & 0.24 & 44.1
FrontKick (200) & 0.097 & 0.19 & 35.2
FrontPunch (213) & 0.081 & 0.39 & 30.1
HighKick (182) & 0.128 & 0.34 & 37.2
HookPunch (200) & 0.122 & 0.32 & 37.4
JumpingJack (200) & 0.122 & 0.28 & 28.2
KneeKick (188) & 0.131 & 0.26 & 37.3
LegBack (208) & 0.158 & 0.30 & 37.9
LegCross (182) & 0.125 & 0.16 & 43.5
RonddeJambe (220) & 0.151 & 0.21 & 39.5
Running (200) & 0.079 & 0.30 & 26.5
Shuffle (198) & 0.088 & 0.20 & 28.3
SideLunges (202) & 0.209 & 0.28 & 46.4
SlowSkater (201) & 0.195 & 0.25 & 42.9
Squat   (205) & 0.185 & 0.24 & 45.3
overall (3000) & 0.140 & 0.27 & 37.3



Pretrainging Mint, 50\% data:

Scratch
Action & RMSE & PCorr & SMAPE
overall (3000) & 0.140 & 0.26 & 38.3
ElbowPunch (201) & 0.140 & 0.25 & 45.0
FrontKick (200) & 0.096 & 0.19 & 36.5
FrontPunch (213) & 0.082 & 0.39 & 31.1
HighKick (182) & 0.129 & 0.34 & 37.9
HookPunch (200) & 0.122 & 0.31 & 38.6
JumpingJack (200) & 0.123 & 0.26 & 29.1
KneeKick (188) & 0.130 & 0.22 & 38.1
LegBack (208) & 0.157 & 0.30 & 38.5
LegCross (182) & 0.126 & 0.15 & 45.0
RonddeJambe (220) & 0.154 & 0.21 & 40.2
Running (200) & 0.080 & 0.29 & 27.3
Shuffle (198) & 0.089 & 0.21 & 29.2
SideLunges (202) & 0.208 & 0.27 & 48.1
SlowSkater (201) & 0.196 & 0.25 & 43.4
Squat   (205) & 0.185 & 0.23 & 46.4
overall (3000) & 0.140 & 0.26 & 38.3

Pret
Action & RMSE & PCorr & SMAPE
overall (3000) & 0.140 & 0.26 & 38.0
ElbowPunch (201) & 0.141 & 0.23 & 44.9
FrontKick (200) & 0.095 & 0.20 & 35.7
FrontPunch (213) & 0.083 & 0.38 & 30.7
HighKick (182) & 0.127 & 0.33 & 38.3
HookPunch (200) & 0.124 & 0.31 & 38.1
JumpingJack (200) & 0.124 & 0.25 & 29.0
KneeKick (188) & 0.128 & 0.23 & 38.2
LegBack (208) & 0.157 & 0.30 & 38.8
LegCross (182) & 0.124 & 0.16 & 44.5
RonddeJambe (220) & 0.152 & 0.21 & 39.8
Running (200) & 0.079 & 0.30 & 27.2
Shuffle (198) & 0.087 & 0.19 & 29.0
SideLunges (202) & 0.212 & 0.27 & 47.8
SlowSkater (201) & 0.198 & 0.25 & 43.3
Squat   (205) & 0.184 & 0.24 & 45.7
overall (3000) & 0.140 & 0.26 & 38.0



Pretrainging Mint, 25\% data:

Scratch
Action & RMSE & PCorr & SMAPE
overall (3000) & 0.141 & 0.24 & 39.4
ElbowPunch (201) & 0.137 & 0.24 & 45.6
FrontKick (200) & 0.096 & 0.17 & 37.5
FrontPunch (213) & 0.084 & 0.35 & 32.6
HighKick (182) & 0.130 & 0.32 & 39.6
HookPunch (200) & 0.127 & 0.30 & 39.8
JumpingJack (200) & 0.122 & 0.26 & 29.0
KneeKick (188) & 0.129 & 0.22 & 39.3
LegBack (208) & 0.159 & 0.28 & 41.2
LegCross (182) & 0.126 & 0.14 & 46.2
RonddeJambe (220) & 0.156 & 0.18 & 41.4
Running (200) & 0.080 & 0.28 & 27.9
Shuffle (198) & 0.090 & 0.19 & 29.6
SideLunges (202) & 0.202 & 0.28 & 49.1
SlowSkater (201) & 0.198 & 0.23 & 44.9
Squat   (205) & 0.187 & 0.24 & 47.7
overall (3000) & 0.141 & 0.24 & 39.4


Pret
Action & RMSE & PCorr & SMAPE
overall (3000) & 0.140 & 0.25 & 39.2
ElbowPunch (201) & 0.142 & 0.24 & 46.2
FrontKick (200) & 0.096 & 0.20 & 37.0
FrontPunch (213) & 0.086 & 0.35 & 31.7
HighKick (182) & 0.132 & 0.33 & 39.2
HookPunch (200) & 0.122 & 0.31 & 39.1
JumpingJack (200) & 0.125 & 0.25 & 30.0
KneeKick (188) & 0.128 & 0.24 & 39.2
LegBack (208) & 0.160 & 0.30 & 39.7
LegCross (182) & 0.125 & 0.15 & 45.3
RonddeJambe (220) & 0.152 & 0.20 & 40.8
Running (200) & 0.081 & 0.30 & 27.5
Shuffle (198) & 0.089 & 0.17 & 29.8
SideLunges (202) & 0.191 & 0.25 & 49.3
SlowSkater (201) & 0.196 & 0.22 & 45.1
Squat   (205) & 0.191 & 0.23 & 47.9
overall (3000) & 0.140 & 0.25 & 39.2


Pretrainging Mint, 12.5\% data:
Scratch

Action & RMSE & PCorr & SMAPE
overall (3000) & 0.142 & 0.23 & 40.7
ElbowPunch (201) & 0.139 & 0.21 & 47.5
FrontKick (200) & 0.093 & 0.16 & 38.3
FrontPunch (213) & 0.087 & 0.33 & 33.5
HighKick (182) & 0.134 & 0.29 & 40.4
HookPunch (200) & 0.123 & 0.25 & 41.9
JumpingJack (200) & 0.128 & 0.24 & 30.7
KneeKick (188) & 0.137 & 0.19 & 41.0
LegBack (208) & 0.155 & 0.27 & 41.4
LegCross (182) & 0.128 & 0.13 & 48.5
RonddeJambe (220) & 0.155 & 0.17 & 42.4
Running (200) & 0.083 & 0.27 & 29.1
Shuffle (198) & 0.090 & 0.16 & 31.6
SideLunges (202) & 0.206 & 0.25 & 51.0
SlowSkater (201) & 0.194 & 0.21 & 46.3
Squat   (205) & 0.191 & 0.22 & 47.6
overall (3000) & 0.142 & 0.23 & 40.7

Pret:
Action & RMSE & PCorr & SMAPE
overall (3000) & 0.141 & 0.23 & 40.6
ElbowPunch (201) & 0.138 & 0.23 & 46.7
FrontKick (200) & 0.094 & 0.18 & 37.7
FrontPunch (213) & 0.087 & 0.36 & 32.4
HighKick (182) & 0.131 & 0.31 & 40.5
HookPunch (200) & 0.125 & 0.27 & 42.2
JumpingJack (200) & 0.125 & 0.23 & 30.7
KneeKick (188) & 0.131 & 0.21 & 40.7
LegBack (208) & 0.160 & 0.27 & 41.6
LegCross (182) & 0.126 & 0.14 & 47.6
RonddeJambe (220) & 0.160 & 0.18 & 43.1
Running (200) & 0.083 & 0.26 & 29.4
Shuffle (198) & 0.091 & 0.15 & 30.6
SideLunges (202) & 0.203 & 0.23 & 51.2
SlowSkater (201) & 0.195 & 0.21 & 46.0
Squat   (205) & 0.190 & 0.23 & 49.3
overall (3000) & 0.141 & 0.23 & 40.6


Pretrainging Mint, 6.25\% data:

Scratch
Action & RMSE & PCorr & SMAPE
overall (3000) & 0.142 & 0.19 & 42.9
ElbowPunch (201) & 0.145 & 0.19 & 49.8
FrontKick (200) & 0.091 & 0.14 & 38.9
FrontPunch (213) & 0.091 & 0.29 & 35.8
HighKick (182) & 0.141 & 0.28 & 43.0
HookPunch (200) & 0.127 & 0.20 & 44.6
JumpingJack (200) & 0.126 & 0.21 & 31.8
KneeKick (188) & 0.131 & 0.18 & 42.8
LegBack (208) & 0.165 & 0.19 & 46.7
LegCross (182) & 0.123 & 0.12 & 48.6
RonddeJambe (220) & 0.159 & 0.17 & 46.2
Running (200) & 0.084 & 0.25 & 29.4
Shuffle (198) & 0.099 & 0.09 & 33.6
SideLunges (202) & 0.189 & 0.21 & 53.0
SlowSkater (201) & 0.190 & 0.18 & 47.0
Squat   (205) & 0.200 & 0.19 & 51.7
overall (3000) & 0.142 & 0.19 & 42.9



Pretrainging Mint, 1\% data:
scratch

Action & RMSE & PCorr & SMAPE
overall (3000) & 0.155 & 0.10 & 51.0
ElbowPunch (201) & 0.145 & 0.11 & 54.7
FrontKick (200) & 0.109 & 0.01 & 51.5
FrontPunch (213) & 0.111 & 0.19 & 47.1
HighKick (182) & 0.153 & 0.11 & 47.7
HookPunch (200) & 0.139 & 0.11 & 53.7
JumpingJack (200) & 0.160 & 0.15 & 41.8
KneeKick (188) & 0.136 & 0.11 & 47.8
LegBack (208) & 0.166 & 0.13 & 51.0
LegCross (182) & 0.126 & 0.06 & 55.6
RonddeJambe (220) & 0.192 & 0.06 & 58.5
Running (200) & 0.114 & 0.14 & 38.2
Shuffle (198) & 0.104 & 0.04 & 39.8
SideLunges (202) & 0.197 & 0.07 & 60.4
SlowSkater (201) & 0.191 & 0.08 & 52.2
Squat   (205) & 0.218 & 0.08 & 63.9
overall (3000) & 0.155 & 0.10 & 51.0

pret

Action & RMSE & PCorr & SMAPE
overall (3000) & 0.151 & 0.11 & 50.0
ElbowPunch (201) & 0.142 & 0.10 & 54.2
FrontKick (200) & 0.098 & 0.08 & 45.4
FrontPunch (213) & 0.120 & 0.15 & 51.1
HighKick (182) & 0.153 & 0.12 & 48.3
HookPunch (200) & 0.135 & 0.11 & 56.3
JumpingJack (200) & 0.147 & 0.13 & 37.6
KneeKick (188) & 0.140 & 0.15 & 47.0
LegBack (208) & 0.176 & 0.10 & 51.9
LegCross (182) & 0.124 & 0.06 & 52.4
RonddeJambe (220) & 0.173 & 0.07 & 57.3
Running (200) & 0.091 & 0.18 & 34.3
Shuffle (198) & 0.097 & 0.05 & 39.7
SideLunges (202) & 0.187 & 0.10 & 60.1
SlowSkater (201) & 0.202 & 0.08 & 53.9
Squat   (205) & 0.208 & 0.13 & 59.1
overall (3000) & 0.151 & 0.11 & 50.0






==> tables/results_mia_2.tex <==
Tranformer Scratch 1
Action & RMSE & PCorr & SMAPE
overall (3000) & 0.158 & 0.09 & 52.9
ElbowPunch (201) & 0.156 & 0.07 & 59.4
FrontKick (200) & 0.104 & 0.07 & 50.8
FrontPunch (213) & 0.127 & 0.10 & 53.8
HighKick (182) & 0.152 & 0.17 & 49.5
HookPunch (200) & 0.162 & 0.07 & 65.0
JumpingJack (200) & 0.159 & 0.12 & 40.8
KneeKick (188) & 0.130 & 0.12 & 47.8
LegBack (208) & 0.178 & 0.10 & 57.1
LegCross (182) & 0.128 & 0.05 & 55.3
RonddeJambe (220) & 0.192 & 0.08 & 60.0
Running (200) & 0.108 & 0.12 & 38.0
Shuffle (198) & 0.105 & 0.06 & 39.2
SideLunges (202) & 0.193 & 0.10 & 60.4
SlowSkater (201) & 0.198 & 0.08 & 55.5
Squat   (205) & 0.215 & 0.11 & 58.9
overall (3000) & 0.158 & 0.09 & 52.9


Transformer Selective Fine-Tune 1 (8% of weight)
Action & RMSE & PCorr & SMAPE
overall (3000) & 0.156 & 0.09 & 54.1
ElbowPunch (201) & 0.155 & 0.06 & 60.8
FrontKick (200) & 0.105 & 0.06 & 52.7
FrontPunch (213) & 0.123 & 0.16 & 54.3
HighKick (182) & 0.156 & 0.13 & 50.8
HookPunch (200) & 0.145 & 0.07 & 61.6
JumpingJack (200) & 0.155 & 0.10 & 40.1
KneeKick (188) & 0.142 & 0.08 & 53.2
LegBack (208) & 0.185 & 0.09 & 61.6
LegCross (182) & 0.120 & 0.07 & 59.0
RonddeJambe (220) & 0.181 & 0.09 & 57.2
Running (200) & 0.097 & 0.15 & 37.9
Shuffle (198) & 0.098 & 0.05 & 40.0
SideLunges (202) & 0.192 & 0.11 & 62.2
SlowSkater (201) & 0.204 & 0.08 & 56.3
Squat   (205) & 0.211 & 0.08 & 62.3
overall (3000) & 0.156 & 0.09 & 54.1



Tranformer Pretrained 1
Action & RMSE & PCorr & SMAPE
overall (3000) & 0.157 & 0.11 & 51.3
ElbowPunch (201) & 0.151 & 0.06 & 58.7
FrontKick (200) & 0.100 & 0.11 & 48.2
FrontPunch (213) & 0.127 & 0.18 & 47.0
HighKick (182) & 0.147 & 0.20 & 49.6
HookPunch (200) & 0.141 & 0.09 & 56.5
JumpingJack (200) & 0.148 & 0.15 & 37.2
KneeKick (188) & 0.138 & 0.12 & 47.6
LegBack (208) & 0.174 & 0.11 & 54.0
LegCross (182) & 0.126 & 0.07 & 55.1
RonddeJambe (220) & 0.187 & 0.06 & 59.2
Running (200) & 0.119 & 0.13 & 40.4
Shuffle (198) & 0.102 & 0.05 & 41.1
SideLunges (202) & 0.206 & 0.12 & 60.1
SlowSkater (201) & 0.193 & 0.10 & 52.5
Squat   (205) & 0.219 & 0.10 & 61.1
overall (3000) & 0.157 & 0.11 & 51.3


Tranformer Scratch 2

Action & RMSE & PCorr & SMAPE
overall (3000) & 0.152 & 0.12 & 49.6
ElbowPunch (201) & 0.155 & 0.08 & 58.8
FrontKick (200) & 0.100 & 0.08 & 46.7
FrontPunch (213) & 0.113 & 0.20 & 46.7
HighKick (182) & 0.145 & 0.17 & 47.6
HookPunch (200) & 0.140 & 0.13 & 52.4
JumpingJack (200) & 0.141 & 0.20 & 35.5
KneeKick (188) & 0.135 & 0.16 & 44.8
LegBack (208) & 0.189 & 0.09 & 58.1
LegCross (182) & 0.124 & 0.09 & 51.5
RonddeJambe (220) & 0.178 & 0.10 & 54.2
Running (200) & 0.117 & 0.08 & 42.3
Shuffle (198) & 0.100 & 0.06 & 38.4
SideLunges (202) & 0.192 & 0.12 & 58.4
SlowSkater (201) & 0.195 & 0.12 & 51.7
Squat   (205) & 0.198 & 0.17 & 55.7
overall (3000) & 0.152 & 0.12 & 49.6

Transformer Selective Fine-Tune 2 (8% of weight)
Action & RMSE & PCorr & SMAPE
overall (3000) & 0.154 & 0.11 & 52.3
ElbowPunch (201) & 0.143 & 0.11 & 57.6
FrontKick (200) & 0.104 & 0.09 & 50.5
FrontPunch (213) & 0.113 & 0.18 & 55.3
HighKick (182) & 0.148 & 0.17 & 51.1
HookPunch (200) & 0.147 & 0.13 & 59.3
JumpingJack (200) & 0.133 & 0.18 & 34.3
KneeKick (188) & 0.138 & 0.10 & 49.5
LegBack (208) & 0.179 & 0.09 & 58.3
LegCross (182) & 0.123 & 0.07 & 58.3
RonddeJambe (220) & 0.162 & 0.10 & 55.7
Running (200) & 0.109 & 0.12 & 39.0
Shuffle (198) & 0.103 & 0.06 & 39.0
SideLunges (202) & 0.218 & 0.10 & 62.9
SlowSkater (201) & 0.187 & 0.08 & 52.5
Squat   (205) & 0.221 & 0.11 & 60.0
overall (3000) & 0.154 & 0.11 & 52.3


Tranformer Pretrained 2
Action & RMSE & PCorr & SMAPE
overall (3000) & 0.151 & 0.13 & 47.9
ElbowPunch (201) & 0.152 & 0.10 & 54.7
FrontKick (200) & 0.098 & 0.11 & 42.3
FrontPunch (213) & 0.101 & 0.20 & 42.1
HighKick (182) & 0.140 & 0.22 & 46.0
HookPunch (200) & 0.138 & 0.16 & 51.5
JumpingJack (200) & 0.138 & 0.16 & 34.8
KneeKick (188) & 0.133 & 0.15 & 46.3
LegBack (208) & 0.174 & 0.12 & 50.9
LegCross (182) & 0.123 & 0.09 & 52.9
RonddeJambe (220) & 0.185 & 0.04 & 55.0
Running (200) & 0.090 & 0.15 & 34.5
Shuffle (198) & 0.107 & 0.06 & 39.2
SideLunges (202) & 0.193 & 0.12 & 58.2
SlowSkater (201) & 0.196 & 0.16 & 49.4
Squat   (205) & 0.212 & 0.13 & 59.6
overall (3000) & 0.151 & 0.13 & 47.9



Scratch 5 
Action & RMSE & PCorr & SMAPE
overall (3000) & 0.148 & 0.17 & 45.1
ElbowPunch (201) & 0.147 & 0.17 & 53.8
FrontKick (200) & 0.096 & 0.11 & 41.3
FrontPunch (213) & 0.098 & 0.26 & 38.9
HighKick (182) & 0.155 & 0.24 & 45.5
HookPunch (200) & 0.129 & 0.17 & 46.1
JumpingJack (200) & 0.132 & 0.19 & 32.5
KneeKick (188) & 0.133 & 0.17 & 44.0
LegBack (208) & 0.177 & 0.15 & 49.4
LegCross (182) & 0.129 & 0.09 & 52.8
RonddeJambe (220) & 0.169 & 0.14 & 48.0
Running (200) & 0.087 & 0.21 & 31.6
Shuffle (198) & 0.096 & 0.12 & 34.6
SideLunges (202) & 0.200 & 0.17 & 55.3
SlowSkater (201) & 0.188 & 0.17 & 49.7
Squat   (205) & 0.200 & 0.17 & 52.6
overall (3000) & 0.148 & 0.17 & 45.1


Fine Tune 5
Action & RMSE & PCorr & SMAPE
overall (3000) & 0.144 & 0.15 & 48.7
ElbowPunch (201) & 0.142 & 0.15 & 54.4
FrontKick (200) & 0.099 & 0.10 & 51.0
FrontPunch (213) & 0.099 & 0.21 & 46.8
HighKick (182) & 0.146 & 0.18 & 48.4
HookPunch (200) & 0.128 & 0.17 & 53.0
JumpingJack (200) & 0.132 & 0.19 & 33.8
KneeKick (188) & 0.129 & 0.15 & 49.0
LegBack (208) & 0.163 & 0.17 & 55.9
LegCross (182) & 0.123 & 0.08 & 57.3
RonddeJambe (220) & 0.155 & 0.13 & 49.1
Running (200) & 0.088 & 0.18 & 32.0
Shuffle (198) & 0.098 & 0.05 & 37.9
SideLunges (202) & 0.203 & 0.18 & 57.5
SlowSkater (201) & 0.194 & 0.14 & 51.8
Squat   (205) & 0.191 & 0.19 & 52.4
overall (3000) & 0.144 & 0.15 & 48.7



Pretrain 5
Action & RMSE & PCorr & SMAPE
overall (3000) & 0.148 & 0.19 & 43.2
ElbowPunch (201) & 0.138 & 0.20 & 49.0
FrontKick (200) & 0.094 & 0.17 & 40.0
FrontPunch (213) & 0.094 & 0.31 & 34.9
HighKick (182) & 0.148 & 0.25 & 43.6
HookPunch (200) & 0.128 & 0.21 & 44.6
JumpingJack (200) & 0.130 & 0.19 & 32.1
KneeKick (188) & 0.134 & 0.18 & 42.8
LegBack (208) & 0.168 & 0.18 & 46.6
LegCross (182) & 0.125 & 0.13 & 49.7
RonddeJambe (220) & 0.171 & 0.13 & 48.6
Running (200) & 0.088 & 0.22 & 30.7
Shuffle (198) & 0.098 & 0.11 & 33.0
SideLunges (202) & 0.220 & 0.19 & 54.4
SlowSkater (201) & 0.195 & 0.19 & 47.8
Squat   (205) & 0.199 & 0.19 & 51.1
overall (3000) & 0.148 & 0.19 & 43.2



Scratch 10
Action & RMSE & PCorr & SMAPE
overall (3000) & 0.144 & 0.21 & 42.0
ElbowPunch (201) & 0.139 & 0.20 & 49.0
FrontKick (200) & 0.096 & 0.18 & 38.6
FrontPunch (213) & 0.089 & 0.30 & 36.9
HighKick (182) & 0.135 & 0.27 & 41.3
HookPunch (200) & 0.125 & 0.26 & 44.6
JumpingJack (200) & 0.131 & 0.23 & 31.4
KneeKick (188) & 0.134 & 0.20 & 41.2
LegBack (208) & 0.163 & 0.25 & 43.6
LegCross (182) & 0.124 & 0.12 & 47.3
RonddeJambe (220) & 0.165 & 0.17 & 45.6
Running (200) & 0.085 & 0.24 & 30.2
Shuffle (198) & 0.092 & 0.13 & 31.5
SideLunges (202) & 0.210 & 0.23 & 50.7
SlowSkater (201) & 0.190 & 0.20 & 47.2
Squat   (205) & 0.197 & 0.21 & 51.1
overall (3000) & 0.144 & 0.21 & 42.0


Fine Tune 10
Action & RMSE & PCorr & SMAPE
overall (3000) & 0.144 & 0.18 & 46.3
ElbowPunch (201) & 0.140 & 0.17 & 53.3
FrontKick (200) & 0.097 & 0.14 & 45.5
FrontPunch (213) & 0.091 & 0.30 & 41.1
HighKick (182) & 0.141 & 0.24 & 45.2
HookPunch (200) & 0.128 & 0.21 & 49.3
JumpingJack (200) & 0.128 & 0.22 & 32.0
KneeKick (188) & 0.137 & 0.13 & 46.7
LegBack (208) & 0.157 & 0.18 & 50.7
LegCross (182) & 0.129 & 0.08 & 56.3
RonddeJambe (220) & 0.161 & 0.13 & 48.5
Running (200) & 0.084 & 0.20 & 31.9
Shuffle (198) & 0.092 & 0.09 & 35.0
SideLunges (202) & 0.197 & 0.20 & 55.9
SlowSkater (201) & 0.200 & 0.18 & 50.5
Squat   (205) & 0.194 & 0.20 & 53.0
overall (3000) & 0.144 & 0.18 & 46.3


Pretrain 10
Action & RMSE & PCorr & SMAPE
overall (3000) & 0.142 & 0.21 & 41.6
ElbowPunch (201) & 0.139 & 0.23 & 47.4
FrontKick (200) & 0.097 & 0.16 & 38.9
FrontPunch (213) & 0.089 & 0.30 & 34.8
HighKick (182) & 0.138 & 0.30 & 41.3
HookPunch (200) & 0.120 & 0.27 & 41.7
JumpingJack (200) & 0.126 & 0.23 & 30.1
KneeKick (188) & 0.129 & 0.19 & 41.5
LegBack (208) & 0.160 & 0.26 & 43.5
LegCross (182) & 0.127 & 0.13 & 47.0
RonddeJambe (220) & 0.157 & 0.14 & 46.5
Running (200) & 0.085 & 0.26 & 29.1
Shuffle (198) & 0.094 & 0.11 & 32.0
SideLunges (202) & 0.200 & 0.20 & 51.9
SlowSkater (201) & 0.193 & 0.20 & 46.2
Squat   (205) & 0.197 & 0.22 & 51.4
overall (3000) & 0.142 & 0.21 & 41.6
